Revisiting Pattern Structure Projections

Formal concept analysis (FCA) is a well-founded method for data analysis and has many applications in data mining. Pattern structures is an extension of FCA for dealing with complex data such as sequences or graphs. However the computational complexity of computing with pattern structures is high and projections of pattern structures were introduced for simplifying computation. In this paper we introduce o-projections of pattern structures, a generalization of projections which defines a wider class of projections preserving the properties of the original approach. Moreover, we show that o-projections form a semilattice and we discuss the correspondence between o-projections and the representation contexts of o-projected pattern structures. KEYWORDS: formal concept analysis, pattern structures, representation contexts, projections

==> tex/paper-template-path.tex <==
\newcommand{\templatepath}{../../../../papers-templates/llncs2e}
